Efficient Parallel Audio Generation using Group Masked Language Modeling

We present a fast and high-quality codec language model for parallel audio generation. While SoundStorm, a state-of-the-art parallel audio generation model, accelerates inference speed compared to autoregressive models, it still suffers from slow inference due to iterative sampling. To resolve this problem, we propose Group-Masked Language Modeling~(G-MLM) and Group Iterative Parallel Decoding~(G-IPD) for efficient parallel audio generation. Both the training and sampling schemes enable the model to synthesize high-quality audio with a small number of iterations by effectively modeling the group-wise conditional dependencies. In addition, our model employs a cross-attention-based architecture to capture the speaker style of the prompt voice and improves computational efficiency. Experimental results demonstrate that our proposed model outperforms the baselines in prompt-based audio generation.

==> compare_tab.tex <==
\begin{table}[th]
\setlength{\tabcolsep}{2pt}
\setlength{\arrayrulewidth}{0.2mm}
\caption{Comparison of the previous systems and SoundOASIS}
\label{tab:multi}
\centering
\begin{tabular}{l l l l}
\toprule
\textbf{Methods} &  \multicolumn{1}{l}{\textbf{AudioLM}}& \multicolumn{1}{l}{\textbf{SoundStorm}}& \multicolumn{1}{l}{\textbf{Sound-OASIS}} \\ 
\midrule
Generative models        & AR & Non-AR & Non-AR  \\
Prompt   & Text and Speech &Text and Speech & Only Speech  \\
Conditioning  & Self-attention &Self-attention& Cross-attention  \\
Inference speed  & Slow & Fast & Very Fast  \\
\bottomrule
\end{tabular}
\end{table}

==> method_orig.tex <==



\begin{figure*} 
\centering
  \includegraphics[width=1.75\columnwidth]{model6_crop.pdf}
  \centering
  \caption{Overall training and sampling procedure are depicted on the left side. Model architecture is depicted on the right side. $s$ denotes the iteration steps.}
  % \vspace{-0.5}
  \label{fig_train}
\label{training}
\vspace{-0.2cm}
\end{figure*}


\section{Proposed method}
\subsection{Tokenization}
We perform $k$-means clustering for semantic tokenization over the 15th hidden representation of Wav2Vec~2.0~\cite{baevski2020wav2vec}. Previous research~\cite {baevski2021unsupervised, kim22c_interspeech} has shown that these discrete tokens effectively capture semantic information, even substituting phonetic sequences. For acoustic tokens, we leverage the bi-group G-RVQ codebooks extracted from HiFi-Codec. Let $\mathbf{x}$ represent a waveform, and $\mathbf{z}\in \mathbb{R}^D$ a latent feature. The acoustic tokenization process is as follows:
\begin{equation}
\label{Acoustic token extraction}
\begin{split}
 \mathbf{z}^{1:D} &= Enc(\mathbf{x})  \\
 [\mathbf{q}^0_0, \mathbf{q}^0_1, \mathbf{q}^1_0, \mathbf{q}^1_1] &= GRVQ(\mathbf{z}),
\end{split}
\end{equation}
where $\mathbf{q}^j_g \in \{1, 2,..., C\}^{T}$ represents the $j$-th quantizer level and $g$-th group of RVQ. The maximum lengths and codebook size are denoted as $T$ and $C$, respectively. Utilizing G-RVQ rather than RVQ can encode sufficient acoustic information even with a reduced RVQ depth, which brings computational efficiency. Subsequently, we set $N_q=2$, making $\mathbf{q}_c=\{\mathbf{q}^0_0, \mathbf{q}^0_1\}$ coarse-grained acoustic codebooks and $\mathbf{q}_f=\{ \mathbf{q}^1_0, \mathbf{q}^1_1 \}$ fine-grained acoustic codebooks.


\subsection{Model Architecture}
As shown in Figure~\ref{training}, our model follows the architecture of SoundStorm~\cite{borsos2023soundstorm}, employing a conformer~\cite{gulati20_interspeech} module and a masked language modeling approach~\cite{devlin2018bert}. Using temporally aligned semantic tokens and acoustic tokens, our model predicts acoustic tokens given the aggregated embeddings of semantic tokens and the corresponding frames of partially masked acoustic tokens. The output embeddings from the prediction network are processed by separate heads for each RVQ level.

To incorporate the speaker and acoustic information of the prompt, we employ a multi-head cross-attention module~\cite{vaswani2017attention} in the prediction network, as shown in Fig.~\ref{fig_train}. 
% The query is derived from the hidden sequence of the self-attention layer, while the key and value are derived from the hidden sequence of the prompt encoder.
Let $\mathbf{z}$ be the output of the prompt encoder and $\mathbf{h}$ be the output of the self-attention in the prediction network. The key, $\mathbf{K}$, and value, $\mathbf{V}$, are derived from the $\mathbf{z}$, and the query, $\mathbf{Q}$ is obtained from the $\mathbf{h}$ through the linear projection layer. 
The multi-head cross-attention module operates as follows:
\begin{equation}
\label{Cross attention}
\begin{split}
 \mathbf{Q}_i = \mathbf{hW}_q^i&,\;  \mathbf{K}_i = \mathbf{zW}_k^i, \; \mathbf{V}_i = \mathbf{zW_v^i}   \\
 \mathbf{head}_i &= Softmax(\frac{\mathbf{Q}_i\mathbf{K}_i}{\sqrt{d}})\mathbf{V}_i\\
 \mathbf{c} &= [\mathbf{head}_1, ..., \mathbf{head}_{N_h}],
\end{split}
\end{equation}
where the $\mathbf{W}^i_q$, $\mathbf{W}^i_k$, and $\mathbf{W}^i_v$ denote the linear projections of the key, value, and query, respectively. The $\mathbf{c}$ represents the context vector summarizing a prompt voice. 
By leveraging the cross-attention mechanism~\cite{vaswani2017attention}, there are distinct advantages compared to the SoundStorm: 
% Firstly, the attention matrix of the cross-attention operates unidirectionally from the prompt to the target sequence, which provides robust conditioning. As a result, our prediction network retains the speaker and acoustic consistency of the prompt embedding, reducing redundant modeling complexity compared to self-attention. 
(1) In contrast to SoundStorm, which mandates semantic tokenization of the prompt sequence, our model efficiently incorporates prompt information using only acoustic tokens. This simplifies the inference process by eliminating the necessity for semantic tokenization of the prompt sequence. (2) Unlike the self-attention structure in SoundStorm, which requires continual computation of the prompt part during the iterative sampling process, our cross-attention mechanism caches the key and value during inference. As a result, the prompt part only needs to be calculated once throughout the entire iterative sampling process, reducing computational redundancy.

\subsection{Training Procedure}
\label{section: training procedure}
Our proposed model is trained following a masked language modeling scheme~\cite{devlin2018bert}. To detail the masking procedure, we begin by randomly selecting the prompt delimiter time step, denoted as $t \sim U\{\epsilon, T-1\}$, where $\epsilon$ is a starting frame constant. The tokens before $t$ constitute the prompt, while those after $t$ form the target sequence for generation. A quantization level indicator parameter $l\in\{0,1\}$ is uniformly sampled to determine the training codebooks. We design the masking strategy based on the G-RVQ properties that the codebooks of different groups with the same quantization level are highly entangled with each other.  

Specifically, when $l=0$, the model predicts coarse-grained codebooks. We apply cosine scheduled mask along the temporal axis to coarse-grained codebooks $\mathbf{q}_c$ while applying mask entire fine-grained codebooks $\mathbf{q}_f$. As cosine masking candidates tokens involve $\mathbf{q}^0_0$ and $\mathbf{q}^0_1$, the model enjoys temporal and group-wise conditional dependency. 
On the other hand, when $l=1$, the focus shifts to predicting fine-grained codebooks. In this scenario, the model applies cosine scheduling masking exclusively to $\mathbf{q}^1_0$ and $\mathbf{q}^1_1$, leaving coarse-grained codebooks $\mathbf{q_c}$ unmasked.  This masking strategy enables the model to leverage RVQ-depth-wise conditional dependency. Given a masked token sequence, we train the model with the cross-entropy loss using the ground-truth acoustic tokens as the target, and the loss is calculated only in the masked locations of tokens.








% \subsection{Speech Prompting}
% To accommodate the variable length of prompt embedding, we employ a cross-attention module, as shown in Fig.~\ref{fig_train}. Let $\mathbf{z}$ be the output of the prompt encoder and $\mathbf{h}$ be the output of the self-attention in the prediction network. The key, $\mathbf{K}$, and value, $\mathbf{V}$, are derived from the $\mathbf{z}$, and the query, $\mathbf{Q}$ is obtained from the $\mathbf{h}$. The multi-head cross-attention module operates as follows:
% \begin{equation}
% \label{Cross attention}
% \begin{split}
%  \mathbf{Q}_i = \mathbf{hW}_q^i&,\;  \mathbf{K}_i = \mathbf{zW}_k^i, \; \mathbf{V}_i = \mathbf{zW_v^i}   \\
%  \mathbf{head}_i &= Softmax(\frac{\mathbf{Q}_i\mathbf{K}_i}{\sqrt{d}})\mathbf{V}_i\\
%  \mathbf{c} &= [\mathbf{head}_1, ..., \mathbf{head}_{N_h}],
% \end{split}
% \end{equation}
% where the $\mathbf{W}^i_q$, $\mathbf{W}^i_k$, and $\mathbf{W}^i_v$ denote the linear projections of the key, value, and query, respectively. The $\mathbf{c}$ represents the context vector. By leveraging the cross-attention mechanism, the model can incorporate prompt information using only acoustic tokens, making the inference process more efficient by eliminating the need for semantic tokenization of the prompt sequence. Furthermore, since the $\mathbf{K}$ and $\mathbf{V}$ are cached during inference, the prompt part only needs to be calculated once during the iterative sampling process, which will be described in the next section.

% To ensure speaker and acoustic consistency, we employ a cross-attention mechanism. In this mechanism, the key and value embeddings are derived from the output of the prompt encoder, while the query embeddings are obtained from the hidden representations of self-attention in the prediction network. There are several advantages to using cross-attention-based speech prompting. 
% Firstly, the model can incorporate prompt information using only acoustic tokens, making the inference process more efficient by eliminating the need for semantic tokenization of the prompt sequence. Secondly, the separate prompt encoder reduces the impact of sequence length on computational complexity, which is otherwise of order $O(n^2)$. Additionally, since the key and value calculated during cross-attention can be reused, the prompt part only needs to be calculated once during the iterative sampling process. Lastly, the cross-attention mechanism better retains conditioning power, especially for short sequences.

\subsection{Group Iterative Parallel Sampling (G-IPD)}
We propose a Group Iterative Parallel Decoding (G-IPD) method for parallel audio generation, which enhances SoundStorm's sampling scheme by additionally modeling group-wise conditional dependency. 

% Our sampling technique leverages the property that the codebooks of different groups with the same quantization level are entangled with each other and exhibit no inherent order. Therefore, our model can operate by expanding the search space by a factor of the number of groups at each iteration.

Our algorithm operates as follows:

%Since our model is trained to predict coarse or fine-grained codebooks regardless of their order, OASIS models the conditional dependency within the coarse or fine-grained codebooks. Our model architecture which consists of parameter-sharing conformer but only different heads facilitate this efficient training. In inference stage, our model samples the tokens in a coarse-to-fine order. By doubling the search space, we expect that the performance degradation is small even if the number of iterations is reduced. 
\begin{itemize}
\item \textbf{Predict} Given the semantic tokens and prompt acoustic tokens, our model predicts the probabilities for all masked locations of $[q_0^0, q_1^0]$.
\item \textbf{Sample} At each masked frame $i$, we sample the token $y_i^{(t)}$ based on its prediction probability. We add the Gumbel noise~\cite{gumbel1948statistical} to the prediction logits for stochastic sampling.
\item \textbf{Rank by Confidence} We regard the prediction logits to be ``confidence" to determine the masked tokens and rank by confidence. In this step, we involve both $[q_0^0, q_1^0]$ codebooks, resulting in doubling the search space, while the original SoundStorm only includes a single codebook.
\item \textbf{Mask} We pick the $k$ lowest confidence tokens and re-mask their tokens. By remaining the high-confidence tokens, our inference models both the group-wise and RVQ-level-wise conditional dependency.  
\end{itemize}
%To support this inference scheme, we propose a masking scheme for training that mimics the inference procedure.

We repeat the above steps for coarse-grained codebooks until the specified number of parallel iterations. For the last iteration, we use greedy decoding rather than confidence-based sampling. Thanks to the RVQ-depth-wise conditional dependency by complete coarse-grained codebooks, the fine-grained codebooks are predicted in a single iteration. These sampling strategies mimic the masked language modeling-based training procedure, as described in Sec.~\ref{section: training procedure}. Notably, the proposed model's performance remains robust even when the number of iterations is reduced by modeling the group-wise conditional dependency.


\label{sec:guidelines}


\begin{algorithm}
  \caption{Group Iterative Parallel Decoding (G-IPD)}
  \label{G-IPD}
  \textbf{Input} model $f_\theta$, target semantic token $\mathbf{c}_s$, prompt acoustic token $\mathbf{c}_a$, masked target acoustic token $\mathbf{q}^{M}_c$, confidence $\mathcal{C}$ \\
  \textbf{Output} predicted target acoustic token $\mathbf{\tilde{q}}_{c}$
  \begin{algorithmic}[1]
      \For{$t \leftarrow \; 0 \; to \; N-1$}
        \State $ y = f_\theta(\mathbf{q}^{M}_{c,t},\mathbf{c}_s, \mathbf{c}_a)$  \Comment{$y$ is predicted logits}
        \State $g \sim Gumbel(0,1)$ 
        \State $y \leftarrow y + \tau \cdot g$  \Comment{Add Gumbel noise to logits}

        \State $\mathbf{q}_{c,t+1} \sim p_{\theta}(\mathbf{q}_{c,t+1}|\mathbf{q}_{c,t}^M, \mathbf{c}_a)$
        \State $p_{\theta}(\mathbf{q}_{c,t+1}|\mathbf{q}_{c,t}^M, \mathbf{c}_a) \leftarrow Softmax(y)$ 

        \State $\mathcal{C} \leftarrow p_{\theta}(\mathbf{q}_{c,t}|\mathbf{q}_c^M, \mathbf{c}_a) $ 
        \State Sample the masking index based on $\mathcal{C}$
        \State $ \mathbf{q}^{M}_{c,t+1}\leftarrow Mask(\mathbf{q}_{c,t})$ \Comment{Cosine scheduled masking}
      \EndFor
\State $\mathbf{\tilde{q}}_c \leftarrow \mathbf{q}_{c,N}$
\State \textbf{return} $\mathbf{\tilde{q}}_c$
  \end{algorithmic}
\end{algorithm}







==> mybib.tex <==
\section*{References}



==> selfcross_tab.tex <==

% \begin{table}
% \caption{Comparison of results for speech prompting method.}
%     \centering
%     \begin{tabular}{|c|c|c|} \hline 
%          &  \multicolumn{2}{|c|}{SECS}\\ \hline 
%  Speech Prompting& Short Prompt&Long Prompt\\ \hline 
%          Self-attention&  3.512& 3.512\\ \hline 
%          Cross-attention&  \textbf{3.812}& \textbf{3.523}\\ \hline
%     \end{tabular}
%     \label{tab:selfcross_tab}
% \end{table}

% \begin{table}[]
% \label{tab1: task}
% \centering
% \caption{Comparison of results for speech prompting method.}
% \begin{tabular}{@{}llll@{}}
% \toprule
% \multicolumn{1}{c}{\multirow{1}{*}{Prompting Methods}}  & \multicolumn{1}{c}{SECS}  &       \multicolumn{1}{c}{RTF}              
% \\ \midrule
% \multicolumn{1}{c}{Self-attention}  & \multicolumn{1}{c}{0.3935} & \multicolumn{1}{c}{0.4231}  \\ 
% \multicolumn{1}{c}{Cross-attention}            & \multicolumn{1}{c}{\textbf{0.4081}} & \multicolumn{1}{c}{\textbf{0.2145}}  \\ 
% \bottomrule
% \end{tabular}
% \end{table}


\begin{table}[]
\label{tab1: task}
\centering
\caption{Comparison of results for speech prompting method.}
\begin{tabular}{@{}llll@{}}
\toprule
\multicolumn{1}{l}{\multirow{1}{*}{Methods}}  &       \multicolumn{1}{c}{RTF}              
\\ \midrule
\multicolumn{1}{l}{SoundStorm} & \multicolumn{1}{c}{0.8231}  \\ 
\multicolumn{1}{l}{\quad \quad \textit{w/o semantic tokenization}} & \multicolumn{1}{c}{0.4145}  \\ 
\multicolumn{1}{l}{Proposed Method} & \multicolumn{1}{c}{\textbf{0.2145}}  \\ 

\bottomrule
\end{tabular}
\end{table}


==> vc_tab.tex <==
\begin{table}[th]
\setlength{\tabcolsep}{2pt}
\setlength{\arrayrulewidth}{0.2mm}
\caption{Comparison of results for zero-shot voice conversion.}
\label{tab:multi}
\centering
\begin{tabular}{l r r r r}
\toprule
\textbf{Method} & \multicolumn{1}{l}{\textbf{CER}}& \multicolumn{1}{l}{\textbf{SECS}}& \multicolumn{1}{l}{\textbf{\quad MOS}}& \multicolumn{1}{l}{\textbf{\; SMOS}} \\ 
\midrule
Ground Truth        & 4.1 & 0.632 & 4.72$\pm$0.06 & 4.65$\pm$0.07  \\
\midrule
VITS   & 6.1 & 0.212 &3.99$\pm$0.10&3.47$\pm$0.09  \\
SoundStorm  & 6.1 & 0.212 &3.99$\pm$0.10&3.47$\pm$0.09  \\
\textbf{Proposed}  & \textbf{6.1} & \textbf{0.212} &\textbf{3.99$\pm$0.10} & \textbf{3.47$\pm$0.09}  \\
\bottomrule
\end{tabular}
\end{table}
